PRSim: Sublinear Time SimRank Computation on Large Power-Law Graphs

{\it SimRank} is a classic measure of the similarities of nodes in a graph. Given a node $u$ in graph $G =(V, E)$, a {\em single-source SimRank query} returns the SimRank similarities $s(u, v)$ between node $u$ and each node $v \in V$. This type of queries has numerous applications in web search and social networks analysis, such as link prediction, web mining, and spam detection. Existing methods for single-source SimRank queries, however, incur query cost at least linear to the number of nodes $n$, which renders them inapplicable for real-time and interactive analysis. { This paper proposes \prsim, an algorithm that exploits the structure of graphs to efficiently answer single-source SimRank queries. \prsim uses an index of size $O(m)$, where $m$ is the number of edges in the graph, and guarantees a query time that depends on the {\em reverse PageRank} distribution of the input graph. In particular, we prove that \prsim runs in sub-linear time if the degree distribution of the input graph follows the power-law distribution, a property possessed by many real-world graphs. Based on the theoretical analysis, we show that the empirical query time of all existing SimRank algorithms also depends on the reverse PageRank distribution of the graph.} Finally, we present the first experimental study that evaluates the absolute errors of various SimRank algorithms on large graphs, and we show that \prsim outperforms the state of the art in terms of query time, accuracy, index size, and scalability.

==> Response.tex <==
\section*{Cover Note for Submission \#411}
We thank the reviewers for the insightful and constructive
comments. We have revised the paper to address the comments, and we
highlight the major changes in {\color{blue} blue} in the revised
paper. Our responses to the reviewers are as follows.


\extraspacing
\noindent\hrulefill \\[-1mm]

\noindent
{\bf \large Meta Reviewer}

\noindent\hrulefill

\extraspacing
\header
{\bf Meta Reviewer, R1:}
{\em Revising the experiments such that that the various algorithms use the same values for shared parameters and by considering a wider range of skewness.}

\header
{\bf Response:} Following the suggestions by each reviewer, we have
made the following efforts  to improve the experiments: 1) We have revised our
experiments so that we can evaluate each algorithm under varying parameters; 2) We
have widened the range of skewness on synthetic datasets; 3) We have
added a sensitivity analysis for parameters $\delta$ and $c$; 4) We have
added experiments on non-power-law datasets; 5) We have added
a scalability analysis for our algorithm. Please see Section 5 for details.

\extraspacing
\header
{\bf Meta Reviewer, R2:}
{\em Correcting the complexity analysis.}

\header
{\bf Response:} We have clarified the concerns about the complexity
analysis. In particular, we have added an algorithm that sorts all
out-adjacency lists according to the in-degrees in $O(m)$
time.  Please see
our response to W1 of Reviewer 5.


\extraspacing
\header
{\bf Meta Reviewer, R3:}
{\em Including results for a fixed target success rate ($1-\delta$, for a user specified $\delta$), rather than $1-1/n$.}

\header
{\bf Response:} We have added the failure probability $\delta$ to
Table~\ref{tbl:intro-compare} and to the
analysis of our algorithm. Please see our response to W3 of Reviewer 1.


\extraspacing
\header
{\bf Meta Reviewer, R4:}
{\em Considering -- at least discussing the impact of-- dynamic data.}

\header
{\bf Response:} We have added the discussion of dynamic graphs to the
paper. Our algorithm is able to support the edge stream model where
edges may be inserted or deleted.  Recall that \prsim generates the
index by performing the backward search 
algorithm on a number $j_0$ of hub nodes. It is shown in~\cite{ZhangLG16} that the results of
the backward search to a
randomly selected target node $w$ can be
maintained with cost $O(k+{\bar{d}\over \e})$, where $k$ is the total number
of insertions/deletions. Since our index stores the results of the backward search
for $j_0$ target nodes, it can process
$k$ insertions/deletions in  $O(kj_0+{m\over \e})$ time. Therefore,
the per-update-cost for processing $k$ updates is bounded by $O(j_0+{m\over \e k})$. However, a thorough investigation of this issue is
beyond the scope of our paper. 



\extraspacing
\header
{\bf Meta Reviewer, R5:}
{\em Reorganizing the paper and clarifying various claims and statements.}

\header
{\bf Response:} We have made the following efforts to re-organize the
paper and to clarify various
claims and statements: 1) We have removed the claim of establishing the
connection between SimRank and PPR; 2) We have removed the power-law
exponent $\beta$ from Section 1 and 2; 3) We have re-organized the
paper so that Section 2 only contains the content required for
understanding Section 3; 4) We have added the theoretical bounds of
PRSim on worst-case graphs to Section 1; 5) We have re-organized
Section 3, 4 and 5 so that we can  decompose the main algorithm into three
key techniques. Each technique is now presented with its analysis,
together with a statement on how it improves
the existing methods, and how it enables PRSim to achieve the desired
time complexity; 6) We have included a discussion on paper~\cite{wang2018efficientsimrank}
mentioned by Reviewer 4. Please see our responses to W1 and  W2 of
Reviewer 1, W1 and W3 of Reviewer 2, W1 of Reviewer 3, D2 of Reviewer 4 and
W1 of Reviewer 5. 


\extraspacing
\header
{\bf Meta Reviewer, R6:}
{\em In particular, the reviewers would like the authors to remove or
  at least re-phrase the claim that they 'discover/establish' the
  connection between simRank and PPR, as reviewers agree that this is
  misleading. It fine to build the proposed method upon this
  relationship, but it would be misleading for the readers if to claim
  that this (establishing the relationship) is one of the main
  contributions of this submission. The reviewers think this will be a
  relatively easy (but important) revision for authors to implement.} 

\header
{\bf Response:} We have removed the claim of establishing the connection
between SimRank and PPR. In fact, this was not our main contribution,
as our estimation formula~\eqref{eqn:formula} can be directly derived by
replacing the hitting probabilities  in SLING's estimation
formula~\eqref{eqn:sling} with $\ell$-hop  RPPR. On the other hand,
our novel contribution is to connect the complexity of SimRank computation
to the reverse {\em PageRank distribution} of the input
graph. In particular, we show that 1) the complexity of our algorithm depends on the
second moment of the reverse PageRank, and 2) the empirical
query time of all existing algorithms also depends on the distribution of
the revers PageRank. To the best of our knowledge, this observation
provides the first quantifiable measure
to the concept of ``locally dense/sparse'' graphs introduced
in~\cite{zhangexperimental}. 



\extraspacing
\noindent\hrulefill \\[-1mm]

\noindent
{\bf \large Reviewer 1}

\noindent\hrulefill

\extraspacing
\header
{\bf Reviewer 1, W1/D4:}
{\em While I appreciate the theoretical formalism, the fact that
  SimRank and PPR are related measures is not a very surprising one.} 

{\em The fact that SimRank and PPR are related is a well known fact:
  simrank on G is known to be equivalent to ppr on $G\times G$.in fact this
  observation was made in the original paper ``G. Jeh and J. Widom.
  Simrank: a measure of structural-context similarity, in KDD,
  2002, pp. 538-543.'' You can see also ``Pei Lee, Laks
  V. S. Lakshmanan, and Jeffrey Xu Yu. 2012. On Top-k Structural
  Similarity Search. In Proceedings of the 2012 IEEE 28th
  International Conference on Data Engineering (ICDE '12)''. }


\header
{\bf Response:} % To the best of our knowledge, there is no rigorous
% connection between SimRank on G and PPR on $G \times G$. First, in both the
% original SimRank paper [15] and Lee's paper [20], we are unable to
% find any claim that explicitly relates SimRank on G to PPR on $G \times G$. In
% particular, [20] states that SimRank on G is similar to PageRank on
% $G \times G$, but emphasizes that the two measures are NOT equal. Secondly,
% based on equation (9) in [15], $s(a,b)$ is the summation of
% probabilities that a sqrt{c}-walk from super-node $(a,b)$ in $G \times G$ FIRST
% visits a singleton super-node $(x, x)$, where the summation is over all
% singleton super-nodes $(x, x)$ (which is only a subset of all
% super-nodes $(a, b)$). Since this definition has the ``first visiting''
% constraint, and the summation is over a subset of all super-nodes, it
% is generally impossible that the SimRank value $s(a,b)$ equals the
% PageRank of super-node $(a, b)$ or the PPR values of $(a,b)$ to any other
% super-nodes in $G \times G$. Finally, even if there is a rigorous connection
% between SimRank on $G$ and PPR on $G \times G$, computing PPR on $G \times G$ will be more
% costly than computing SimRank on G, due to the tremendous amount of
% nodes and edges in $G \times G$.  
We have removed the claim of establishing the connection
between SimRank and PPR. In fact, this was not our main contribution,
as our estimation formula~\eqref{eqn:formula} can be directly derived by
replacing the hitting probabilities  in SLING's estimation
formula~\eqref{eqn:sling} with $\ell$-hop  RPPR. On the other hand,
our novel contribution is to connect the complexity of SimRank computation
to the reverse {\em PageRank distribution} of the input
graph. In particular, we show that 1) the complexity of our algorithm depends on the
second moment of the reverse PageRank, and 2) the empirical
query time of all existing algorithms also depends on the distribution of
the revers PageRank. To the best of our knowledge, this observation
provides the first quantifiable measure
to the concept of ``locally dense/sparse'' graphs introduced
in~\cite{zhangexperimental}. 



\extraspacing
\header
{\bf Reviewer 1, W2/R2:}
{\em The paper is poorly written. Many of the key concepts, such as
  $\beta$, are used before they are properly introduced, which makes it
  confusing (for example, in Page 2 authors state that the power law
  distribution exponent, $\beta$, takes values between 0 and 1 -- and
  only later in Section 2-- they explain that $\beta$ is $1/\gamma$, where
  $\gamma$ is the traditional power-law exponent). Also, significant
  parts of the paper reads like a survey, and the key contribution
  comes only after Page 5.}  

{\em Re-organize the content so that the key concepts are introduced
  sufficiently early and the key ideas are presented before page 6.}

\header
{\bf Response:} Thank you for this insightful advice. We have removed
$\beta$ from Section 1 and Section 2 in the revised paper. We have also re-organized the paper so that
Section 2 only contains the content required for understanding Section
3.  


\extraspacing
\header
{\bf Reviewer 1, W3/R1:}
{\em Why $1-1/n$ is a meaningful success probability in Definition 1?
  Why not $1-1/sqrt(n)$ or $1-1/log(n)$? For large values of $n$, seeking a
  success probability of $1-1/n$ seems rather meaningless. For example,
  the MC based "ground truth" used in the experiments are designed for
  success probability $1/1000$, which would be *less than* $sqrt(n)$ for
  all  the data sets considered here. Also prior work, such as [25],
  defines success rate as $1 - \delta$, not $1- 1/n$. How would the
  performance results in Table 1 (for PRSim and other algorithms)
  change if the success probability is fixed at $1- \delta$ rather than
  being an unrealistic target, $1-1/n$?}

{\em Fix Table1. Also, include results for a fixed target success rate
  ($1-\delta$, for a user specified $\delta$), rather than $1- 1/n$. }

\header
{\bf Response:} We have changed the target success probability from $1-1/n$
to $1-\delta$ (See
Table~\ref{tbl:intro-compare}). For
TSF, READS, ProbeSim, this changes their query bounds from
$O\left({{n\over \e^2} \log n }
             \right)$ to $O\left({{n\over \e^2} \log {n \over \delta} }
             \right)$.  Note that there is still a factor of $n$ in the
logarithm, as these algorithms need to apply the union bound on $n$ nodes
to ensure a success probability of $1-\delta$ for a single-source query.  




\extraspacing
\header
{\bf Reviewer 1, D1:}
{\em Table 1 needs to be revised: please add a column indicating the
  key assumptions (for example PRSim assumes power-law graphs); also
  it looks like the space and time overhead of the various algorithms
  need to also include the term "$m$".}

\header
{\bf Response:} We have added the query cost of \prsim on worst-case
graphs to Table~\ref{tbl:intro-compare}. The space and time overhead
of TSF and READS do not depend on the number of edges $m$;
they generate a fixed number of $\scw$-walks from each node of the graph,
and the cost of generating a single $\scw$-walk is a constant. 

\extraspacing
\header
{\bf Reviewer 1, D2:}
{\em The experimental evaluation lacks parameter sensitivity analysis
  for decay factor "$c$", error parameter "$\epsilon$" (and target success
  rate!).}

\header
{\bf Response:} We have revised our experiments so that we can
evaluate \prsim with varying error parameter $\e$. We have also added sensitivity analysis for decay factor
$c$ and target success rate $1-\delta$. 



\extraspacing
\header
{\bf Reviewer 1, D3/R3:}
{\em Also, authors claim that they have set the competitors'
  parameters to the values recommended in the corresponding
  articles. For instance, the $\epsilon$ parameter for ProbeSim is set
  to $0.1$ "as suggested in [25]." This is, however, not strictly
  correct. [25] does not *recommend* $\epsilon$ parameter to be set to
  $0.1$. Given that both PrSim and ProbeSim have this parameter, it
  would have made sense that they were set to the same values ($0.05$
  and $0.2$) for fair comparison. Otherwise, I am not sure the results
  in Figures 2 through 6 makes sense.}

{\em Please justify your selection of the parameters for
  competitors. Most importantly, revise the experiments, such that
  that the various algorithms use the same values for shared
  parameters. }

\header
{\bf Response:} Following your suggestion, we have revised our
experiments so that we can  evaluate each algorithm with varying parameters. The
experiments show that our algorithm outperforms the competitor in
terms of the tradeoffs between accuracy and space/time
complexity. Please see Section 5 for details.





\extraspacing
\noindent\hrulefill \\[-1mm]

\noindent
{\bf \large Reviewer 2}

\noindent\hrulefill

\extraspacing
\header
{\bf Reviewer 2, W1/D2:}
{\em I found confusing the first two contributions; as I found that
  these two contributions overlap. Is nt the algorithm based on the
  connection between pagerank and simrank. }

{\em   Please verify if contribution 1 and 2 overlap or otherwise
  explain better.}

\header
{\bf Response:} % We believe that the two contributions do not
% overlap. For the first contribution, we use the connection between
% SimRank and PPR to derive a sub-linear time algorithm. For the second
% contribution, we focus on the hardness of the SimRank problem and
% conduct experiments to show that the query performance of ALL SimRank
% algorithms is closely related to the PageRank distribution of the
% graph.
% That said, w
We agree that the original claims may lead
to misunderstanding. We have revised the contribution part according
to your suggestion. In particular, we have removed the claim of
establishing the connection
between SimRank and PPR, and  added a detailed explanation on how PRSim extends
  existing SimRank and PPR methods. Please see  the ``our
  contributions'' part
  in Section 1. 





\extraspacing
\header
{\bf Reviewer 2, W2:}
{\em Are the datasets used (table 3) power-law graphs? It would be
  interesting to see the behavior of the algorithm on known (or
  synthetic) non power law graphs! }  

\header
{\bf Response:} We have added the time complexity of our algorithm on
worst-case graphs to Table~\ref{tbl:intro-compare}. Our algorithm runs in $O\left({n\log {n\over \delta}  \over \e^2} \cdot
  \sum_{w \in V} \pi(w)^2 \right)$ on worse-case graphs, where $
\sum_{w \in V} \pi(w)^2 $ is the second moment of the reverse
PageRank. By the fact that $\sum_{w\in V} \pi(w)^2  \le \left(\sum_{w\in V} \pi(w)\right)^2 = 1$,
  \prsim provides at least the same complexity as random walk based
  algorithms (ProbeSim, TSF, and READS) do on worst-case
  graphs. Furthermore, even if the input graph is not a power-law graph, it is still
  possible that the second
  moment $\sum_{w\in V} \pi(w)^2$ is significantly less than $1$, in
  which case \prsim also outperforms existing methods. 
 
On the empirical aspect, most real-world graphs follow  distributions
that are at least close to the power-law distribution. Therefore, we have added experiments
on synthetic non-power-law graphs according to your suggestion. 





\extraspacing
\header
{\bf Reviewer 2, W3:}
{\em  Is section 2 too long?}  

\header
{\bf Response:} We have re-organized the paper so that
Section 2 only contains the content required for understanding Section
3.  



\extraspacing
\header
{\bf Reviewer 2, W4:}
{\em  I am wondering if this time improvement is really necessary, since these scores can also pre-computed.}  

\header
{\bf Response:} As we mentioned in Section 1, it is not feasible to
pre-compute SimRank values for large graphs  as it requires
$\Theta(n^2)$ space. For example, for a 
graph with $n=10^7$ nodes, we need to store  $10^{14}$ float numbers,
which takes 400 terabytes of space. 



\extraspacing
\header
{\bf Reviewer 2, D1:}
{\em   In Abstract the sentence: ``To the best of our knowledge, this
  is the first sublinear algorithm for single-source SimRank queries.''
  Does this sentence refer to all graphs or only when power law is
  around! Please verify.}   

\header
{\bf Response:} The sub-linear query
bounds only work for power-law graphs. Note that
it is impossible to achieve sub-linear query time on worst-case
graphs. Specifically, consider the following star-shaped graph: node 1
is connected to node $2, 3, \ldots, n$, and there are no other
edges. Consider a single-source query for node 2. It is easy to see
that  
the SimRank values $s(2, 3) = s(2, 4) =\ldots = s(2, n) = c$. This means the
output size of the single-source query is already $\Omega(n)$, even if we
allow constant error.  

On the other hand, we have added analysis that shows our algorithm runs in $O\left({n\log {n\over \delta}  \over \e^2} \cdot
  \sum_{w \in V} \pi(w)^2 \right)$ on worse-case graphs.  Since
$\sum_{w \in V} \pi(w)^2 $ can be significantly smaller than $1$ on
non-power-law graphs, our algorithm still outperforms existing methods
on worst-case graphs. 

\extraspacing
\noindent\hrulefill \\[-1mm]

\noindent
{\bf \large Reviewer 3}

\noindent\hrulefill

\extraspacing
\header
{\bf Reviewer 3, W1/D1/D2:}
{\em   Algorithms and the analysis in the paper are hard to follow,
  and the current version of the manuscript does not provide an
  intuitive explanation on how and why existing methods are extended,
  and what are the novel contributions of the proposed approach? (See
  D1 and D2)}

{\em PRSim draws the connection between SimRank and Personalized
  PageRank (reverse PPR in particular) and exploits the skewness of
  the graph to minimize the cost of RPRR estimations, which leads to
  sublinear query time for SimRank with proper indexing
  structures. Novel contributions of PRSim is to re-formulate random
  walk based definition of SimRank in terms of RPRR and to utilize
  skewed PR distribution of the graph for selective indexing. However,
  these are not clear in the Section 1. I believe that Section 1 and 2
  can be re-organized to clearly state: (i) how and why PRSim extends
  existing SimRank and PPR methods, and (ii) what are the novel
  contributions that enable PRSim to outperform its competitors.}

{\em Algorithms and the analysis presented in the current version
  of the manuscript are hard to follow, do not provide an intuitive
  explanation and make it harder to distinguish the specific
  contributions of the proposed approach. Therefore, my recommendation
  is to re-organize section 4 and 5 in a way that each algorithm and
  analysis is presented together, combined with an intuitive
  explanation on why the particular techniques and modifications are
  used.}

{\em W1 can be addressed by D1 and D2.}

\header
{\bf Response:} Thanks for this insightful advice. We have
re-organized the paper according to your suggestions. In particular,
we have made the following changes to the paper: 1) We have added
the theoretical bounds of \prsim on worst-case graphs to Section 1; 2)
We have clearly stated how PRSim extends
  existing SimRank and PPR methods, and how the techniques enable
  PRSim to outperform its competitors.  Please see contribution 2 in
  Section 1.  3) We have re-organized
Section 3, 4 and 5 so that we can  decompose the main algorithm into three
key techniques. Each technique is now presented with its analysis,
together with a statement on how it improves
the existing methods, and how it enables PRSim to achieve the desired
time complexity.




\extraspacing
\header
{\bf Reviewer 3, W2/D5/R2:}
{\em  Limited experimental evaluation in terms of the skewness of the
  graphs. Although many real-world graphs are known to fit into the
  skewness assumption that authors make, it is important to consider a
  wider range of skewness for the sake of completeness. (See D5)}     

{\em Authors use the parameter values that are specified in the
  original papers for other methods. Although I believe that it is
  extremely important to be able to replicate the results of original
  studies, I believe that it is misleading to compare algorithms with
  different parameters. For instance, error parameters affect the
  run-time cost of all algorithms and therefore I believe that results
  might have looked differently under a fair comparison.}



{\em W2 and W3 can be addressed by D5, D7 and D8. In general, it
  is necessary to provide more detailed and comprehensive empirical
  evidence. First of all, using same parameter setting for all
  algorithms in addition to Section 6.2 would provide a fair basis for
  the experimental evaluation (same error parameters, or setting the
  random walk depth l as same as READS's random walk depth t
  etc.). Second, it is not clear how parameters of PRSim is selected,
  it is important to clearly specify and justify parameter selection
  for the proposed algorithm, ideally combined with a sensitivity
  analysis. }


\header
{\bf Response:} Following your suggestion, we have revised our
experiments so that we can evaluate each algorithm under varying parameters. The
experiments show that our algorithm outperforms the competitor in
terms of the tradeoffs between accuracy and space/time
complexity. Please see Section 5 for details.



\extraspacing
\header
{\bf Reviewer 3, W3/D7/D8:}
{\em  Selection of the parameters in the experimental setup is not clear (See D7 and D8)}    

{\em What are the power-law exponents of the real-world graphs used in
  the experiments? Synthetic datasets with variable power-law
  exponents enables us to understand the impact of skewness the query
  performance. However, only $\gamma$ values used in Section 6.4 are in
  [1,2] range (to comply with the skewness assumption in Section 4). I
  believe it is important to extend the experiments in Section 6.4 to
  cover a wider range of $\gamma$ for sake of completeness. }

{\em What are the parameters c and l that are used in Section 6?}



\header
{\bf Response:} We have widened the choice of $\gamma$ to $[1,
9]$. Note that existing power-law graph generator are only able to
generate power-law graphs with $\gamma\ge 1$. Please see
Section 5 for a detailed evaluation.  We set the decay factor $c$ of SimRank to 0.6, in line
with previous work \cite{MKK14,Yu13,LVGT10,YuM15a,YuM15b}. We have
also added a sensitivity analysis on $c$. 

\extraspacing
\header
{\bf Reviewer 3, D3/D4:}
{\em  Algorithm 2: Condition in Line 16 is different from the one described on Page 7.}    

{\em Algorithm 5: I believe the condition in Line 13 refers to the residue of a vertex, not the l-hop RPRR.}

\header
{\bf Response:} Corrected as advised.






\extraspacing
\header
{\bf Reviewer 3, D6:}
{\em  Many real-world graphs are dynamic, and therefore efficient
  index maintenance under the edge-stream model is an important
  feature for real-world applications. I believe it would be an
  important contribution if authors can at least discuss the cost of
  index maintenance.}     

\header
{\bf Response:} We have added a brief discussion on how to support
the edge-stream model where edges may be inserted or deleted.  Recall that \prsim generates the
index by performing the backward search 
algorithm. It is shown in~\cite{ZhangLG16} that the results of
the backward search to a
randomly selected target node $w$ can be
maintained with cost $O(k+{\bar{d}\over \e})$, where $k$ is the total number
of insertions/deletions. Since our index stores the results of the backward search
for $j_0$ target nodes, it can process
$k$ insertions/deletions in  $O(kj_0+{m\over \e})$ time. Therefore,
the per-update-cost for processing $k$ updates is bounded by $O(j_0+{m\over \e k})$.   However, a thorough investigation of this issue is
beyond the scope of our paper. 


\extraspacing
\header
{\bf Reviewer 3, D9:}
{\em  Current version of the manuscript contains many typos and requires language editing.}     


\header
{\bf Response:}  We have done a careful pass of the paper and fixed many presentation issues in the
paper.






\extraspacing
\noindent\hrulefill \\[-1mm]

\noindent
{\bf \large Reviewer 4}

\noindent\hrulefill

\extraspacing
\header
{\bf Reviewer 4, W1:}
{\em   While most of the major competitors in the paper, i.e., READS,
  TSF and ProbSim, are mainly designed to handle dynamic graphs, the
  PRSim algorithm can only deal with static graphs. When the graph is
  updated, it needs to re- compute the whole index, which limits the
  scope of the proposed algorithm.}    

\header
{\bf Response:}  First of all, our algorithm is able to support dynamic
graphs where edges may be inserted or deleted.  Recall that \prsim generates the
index by performing the backward search 
algorithm on a number $j_0$ of hub nodes. It is shown
in~\cite{ZhangLG16} that the results of the backward search to a
randomly selected target node $w$ can be
maintained with cost $O(k+{\bar{d}\over \e})$, where $k$ is the total number
of insertions/deletions. Since our index stores the results of the backward search
for $j_0$ target nodes, it can process
$k$ insertions/deletions in  $O(kj_0+{m\over \e})$ time.   Therefore,
the per-update-cost for processing $k$ updates is bounded by
$O(j_0+{m\over \e k})$.  We
have added this discussion to the paper. 


Besides, many existing
IT companies, such as Pinterest~\cite{eksombatchai2018pixie} and
Twitter~\cite{gupta2013wtf},
are periodically updating the graph for graph
queries instead of always using the up-to-date graph.  We would like
to pinpoint that our index scheme will be still beneficial in such
scenarios. For example, on the billion-edge dataset Twitter, when providing the same additive error of
$10^{-3}$, READS can process around
8,000 queries per day. However, our PRSim can process more than
140,000 queries per day.  Meanwhile, PRSim can rebuild its index on
Twitter in less than 300 seconds, which is an acceptable cost for most applications.



Finally, to ensure a fair comparison, we only compare our
algorithm to the static version of READS, which is the fastest among
the three variants ~\cite{jiang2017reads}. On the other hand, TSF and
ProbeSim suffer from some drawbacks when processing large graphs. TSF always overestimates the
actual SimRank values, and thus is unable to achieve high precision in
our experiments. ProbeSim, on the other hand, is unable to achieve
high precision using a reasonable amount
of query time on hard graphs such as Twitter. Therefore, we believe
indexing is still useful if we need high accuracy on large graphs. 


% an index-free algorithm and thus is
% most flexible. However, our experiments show
% that indexing is actually useful for hard dataset such as Twitter, on which
% ProbeSim is unable to 







\extraspacing
\header
{\bf Reviewer 4, W2/D3:}
{\em    In experiments, the query time, indexing time and index size
  under different parameters (e.g., error bound, power- lar
  parameter, failure probability) of different algorithms should be
  tested, instead of only varying data sets.}    

{\em More experiments should be added, the indexing time and index
  size of different algorithms under different power- law parameters,
  in addition to the query time, to verify the efficiency and
  scalability of the proposed algorithm.}

\header
{\bf Response:} Following your suggestion, we have revised our
experiments so that we can evaluate each algorithm with varying parameters. The
experiments show that our algorithm outperforms the competitors in
terms of the tradeoffs between accuracy and space/time
complexity. Please see Section 5 for details.


% However, varying parameters for various
% algorithms is a not practical approach for conducting experiments on
% large graphs with
% limited time. For example, the preprocessing time of SLING exceeds 24
% hours for any error parameter $\e < 0.1$ on datasets larger than WB;
% READS runs out of 196 GB memory if we increase $r$  from the default
% value $100$ to $200$ on datasets larger than TW. TSF also suffers the
% same issue as we increase the number of one-way graphs $R_g$  stored in
% the index.

% Therefore, we propose the following alternative: we fix
% parameters of the competitors and vary the parameter
% $\e$ of our algorithm to plot a curve that indicates the tradeoff
% between the error and query
% time. If our algorithm is able to achieve lower error with less query
% time, we can safely conclude that our algorithm ``dominates'' the
% competitors in terms of accuracy-query time tradeoffs. We can perform
% similar experiments for index size, index time and precision of
% top-$k$ results. This approach has been widely used in~\cite{liu2017probesim}



\extraspacing
\header
{\bf Reviewer 4, W3:}
{\em  The authors should provide theoretical guarantee for relative
  error for Top-k results instead of absolute additive error, as
  TopPPR and FORA mentioned in the paper. In practice, it is important
  to consider the orders of the top-k results not the scores.}     

\header
{\bf Response:} Unlike the work on PPR, all existing SimRank
algorithms only consider the absolute
additive error. The reason is that
computing SimRank is significantly harder than computing PPR. In
particular, consider a simple Monte Carlo algorithm that answers a
single-source PPR query from source node $u$. We generate a
number $n_r$ of random walks from $u$, and use the fraction of random
walks that terminate at $w$ to estimate the PPR value $\pi(u,w)$. If we set $n_r =
O(\log {n\over \delta} /\e^2)$, we can estimate each PPR value $\pi(u,
w)$ with absolute additive error $\e$, with probability at least
$1-\delta$; If we set $n_r =
O(n\log {n\over \delta} /\e^2)$, we can estimate each PPR value $\pi(u,
w)$ with relative error $\e$, with probability at least
$1-\delta$, for any $\pi(u, w) > 1/n$. 


However, if we want to answer a single-source SimRank
query from node $u$ using the Monte Carlo algorithm, we need to generate $n_r$  random walks from EACH node in the
graph. Therefore, the cost of estimating each SimRank value $s(u,v)$
with absolute additive error $\e$ is already $O(n\log {n\over \delta}
/\e^2)$. If we want a relative error of $\e$ for any $s(u,v) > 1/n$,
the complexity will boost up to $O(n^2\log {n\over \delta}
/\e^2)$, which is unacceptable for large graphs. 

Finally, we have also included an experiment that evaluates the
precision of top-k results of each algorithm. The result shows that
our algorithm outperforms the competitors by obtaining a higher
precision using less query cost.



\extraspacing
\header
{\bf Reviewer 4, D2:}
{\em  The authors claim in introduction and related works that all
  pair SimRank computation requires $O(n^{2})$ space, however, it has
  been recently shown that this space cost can be reduced and
  determined by the graph density and error bound. (ICDE'18).}     

\header
{\bf Response:} Thanks for pointing this out. We have
cited~\cite{wang2018efficientsimrank} in the revised paper.
\cite{wang2018efficientsimrank} reduces the $O(n^2)$
space cost to $O(NNZ)$, where $NNZ$ is
the number of node pairs with large SimRank similarities. However,
$NNZ$ can be as large as $n^2$ on worst-case graphs. Specifically, consider the following star-shaped graph: node 1
is connected to node $2, 3,\ldots , n$, and there are no other
edges. It is easy to see that for any node pair $(i,j)$, $i \neq j \ge
2$, we have $s(i, j) = c$, and thus $NNZ  \ge (n-1)(n-2)$. 

On the other hand, it was 
shown in~\cite{wang2018efficientsimrank} that even on real-world graphs,
$NNZ$ can be as large as $0.06\cdot n^2$ for reasonably small error bound $\e$. This complexity is still unaffordable for
large graphs where $n$ can be as large as $10^{10}$.









\extraspacing
\header
{\bf Reviewer 4, D4:}
{\em There are some topos, e.g.., $\pi_{l}(u,w)$ above Eq.(5) should be
  involved in a summation, and $n\pi(w)$ below Eq.(7) should be $n\pi(x)$.}     

\header
{\bf Response:} We have done a careful pass of the paper and fixed many presentation issues in the
paper.



\extraspacing
\header
{\bf Reviewer 4, D5:}
{\em  In section 2.3, the authors challenge the pre-processing time of
  Sling, however, the indexing time for online query is performed
  off-line, which is acceptable. Besides, as stated in Sling, the
  index phases can be executed in parallel.}      

\header
{\bf Response:} The preprocessing time of SLING is significantly
higher than that of the competitors, which is an issue even with
parallelism. First of all, the preprocessing time matters  if we want  to apply SLING on dynamic
graphs, in which case we need
to recompute its index periodically to reflect the changes of the
graph. Second, 
the preprocess algorithms of TSF, READS, and
TSF can also be executed in parallel. Our algorithm can also be
trivially parallelized: we simply run the backward search algorithm on
multiple hub nodes. Therefore, running in parallel does not give SLING
an advantage over the competitors. Finally and most importantly, SLING
spends most (99.9\%) of its
preprocessing time on estimating the last meeting probability
$\eta(w)$ for each $w\in V$. One of the key insight in our paper is
that this time-consuming part is actually redundant, as
we can estimate $\eta(w)$ in the query phase without increasing the
asymptotic query cost. Therefore, our technique also improves the
preprocessing time of SLING. 






\extraspacing
\noindent\hrulefill \\[-1mm]

\noindent
{\bf \large Reviewer 5}

\noindent\hrulefill

\extraspacing
\header
{\bf Reviewer 5, W1/D1/R1:}
{\em   The complexity analysis of preprocessing is not correct.}

{\em  The authors conclude the complexity of pre-processing is
  linear w.r.t  number of edges. However, the time complexity of sorting the
  out adjacency list of every node (lines 1-2 in Algorithm 5) is not
  considered. Even worse, doing sorting is always time-consuming
  especially when a node has $n$ neighbors, which further leads to
  $O(nlog n)$ complexity. }

{\em Revise the complexity analysis of pre-processing.}

\header
{\bf Response:} Thanks for pointing this out. Sorting adjacency lists
according to an arbitrary order function
is indeed time-consuming. However, in our preprocessing algorithm, we sort
the out-adjacency list of
each node according to the in-degrees, which can be done in time
linear to $m$. More precisely, we first construct a
tuple $(u,v, \din(v))$ for each edge $(u,v) \in E$. Then we employ
the {\em counting sort} algorithm to sort the
$m$ tuples $(u,v, \din(v))$ according the ascending order of
$\din(v)$. Since $\din(v)$ is an integer in  $[0,n]$,
the counting sort algorithm runs in time $O(m+n)$. We then scan the $m$ sorted
tuples and, for each tuple $(u,v, \din(v))$, we append $v$ to the end
of $u$'s out-adjacency list. This algorithm sorts all out-adjacency
lists in $O(m+n)$ time.  We have added above discuss the
paper, and have modified Algorithm~\ref{alg:indexing} accordingly.




\extraspacing
\header
{\bf Reviewer 5, W2/D4/R2:}
{\em No scalability experiments are conducted to verify the sub-linear query complexity.}
{\em   Scalability experiments (i.e., query time vs. the size of network) to demonstrate the sub-linear complexity.} 

\header
{\bf Response:} We have added scalability experiments to demonstrate
the sub-linear complexity.





\extraspacing
\header
{\bf Reviewer 5, W3/D2:}
{\em Details of the algorithm are missed (e.g., how to choose the parameters).}
{\em    Throughout the paper, there are lots of 'magic numbers' (e.g.,
  line 1 in Algorithm 2) without explanations how to get these
  numbers.} 

\header
{\bf Response:} We have added explanations on how and why we use these
numbers. Please see Section 3 for details.



\extraspacing
\header
{\bf Reviewer 5, D3:}
{\em     In line 10 of Algorithm 1, r.h.s should be $\eta\pi_l(u,w)$.}

\header
{\bf Response:} Revised as advised.







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

